How Do We Engage with Other Disciplines? A Framework to Study Meaningful Interdisciplinary Discourse in Scholarly Publications

With the rising popularity of interdisciplinary work and increasing institutional incentives in this direction, there is a growing need to understand how resulting publications incorporate ideas from multiple disciplines. Existing computational approaches, such as affiliation diversity, keywords, and citation patterns, do not account for how individual citations are used to advance the citing work. Although, in line with addressing this gap, prior studies have proposed taxonomies to classify citation purpose, these frameworks are not well-suited to interdisciplinary research and do not provide quantitative measures of citation engagement quality. To address these limitations, we propose a framework for the evaluation of citation engagement in interdisciplinary Natural Language Processing (NLP) publications. Our approach introduces a citation purpose taxonomy tailored to interdisciplinary work, supported by an annotation study. We demonstrate the utility of this framework through a thorough analysis of publications at the intersection of NLP and Computational Social Science.

==> latex/unused_model.tex <==
% \section{Automatic Citation Purpose Classification}
\section{Experiments}
In this section, we discuss model details and evaluations of the automatic components of the framework described in Section \ref{sec:framework}.

\subsection{Track Classifier}
To build our binary track classifier, we fine-tune RoBERTa base \cite{gururangan-etal-2020-dont} with the labeled abstracts using HuggingFace's Transformers Trainer \cite{wolf2020huggingfacestransformersstateoftheartnatural}. To account for class imbalance, we used weighted cross entropy loss. The learning rate was set to $2e-5$ and we trained for 50 epochs. We used a training split of 80\% of the labeled data, a validation split of 10\% and a test split of 10\%. The model which obtained the maximum Macro F1 score on the validation set was loaded at the end of training and obtained a Macro F1 score of 0.870 on the test set. A more detailed breakdown of the model performance may be found in Appendix \ref{app:track_classifier_details}.

% \subsection{Claim Extractor}
% - Fine-tuned RoBERTa large to extract article claims from the abstract
    
%     - lr = 3e-5
    
%     - batch size = 16
    
% - Trained on 1500 biomedical article dataset released by \citet{achakulvisut2020claimextractionbiomedicalpublications}

% - Performed classification at the sentence-level, with the previous sentence for context. 

% - Performance on biomed data: 0.9 F1, 5-fold validation

% - Final trained model used for our data contains 4552 sentences, split equally amongst claims and non-claims



\subsection{Citation Purpose Classifier}
task, model details, prompts
discuss results, include table with all model configs
% \paragraph{Dataset} Define dataset that we use to perform evaluation (NLP papers) and experimental settings ... 

% I think we need to do a bit of labeling or post-hoc analysis on in-domain data to see how well we do things.

% \begin{itemize}
%     \item Can we correctly identify the sub-field of the source paper? 
%     \item Can we correctly identify the discipline of the cited paper?
%     \item Can we correctly identify arguments?
%     \item Can we correctly identify argument roles?
%     \item Can we correctly identify relations? 
% \end{itemize}
